Every Feedforward Neural Network Definable in an o-Minimal Structure Has Finite Sample Complexity

We show that, in a precise sense, a broad class of feedforward neural networks learn (have finite sample complexity) in the PAC model: every fixed finite feedforward architecture whose layers are definable in an o-minimal structure has finite sample complexity in the agnostic PAC setting, even with unbounded parameters. This covers standard fixed-size MLPs, CNNs, GNNs, and transformers with fixed sequence length, together with the operations and layers typically used in such architectures, including linear projections, residual connections, attention mechanisms, pooling layers, normalization layers, and admissible positional encodings. Hence, distribution-free learnability for modern non-recurrent architectures is not an exceptional property of particular activations or architecture-specific VC arguments, but a consequence of tame feedforward computation. Our results reposition finite-sample PAC learnability as a baseline rather than a differentiator: they shift the focus of architectural comparison toward inductive biases, symmetries and geometric priors, scalability, and optimization behaviour.

==> Bookkeeping/0_AuthorsandInfo.tex <==
% \title{Decentralization Can Break The Curse of Dimensionality}
% \author{Anastasis Kratsios, Marc T. Law, Haitz Sáez de Oc\`{a}riz Borde, and Takashi Furuya}
% \date{October 2023}


% \title[Decentralization Breaks The Curse of Dimensionality]{Decentralization Breaks The Curse of Dimensionality}
% \usepackage{times}
% % Use \Name{Author Name} to specify the name.
% % If the surname contains spaces, enclose the surname
% % in braces, e.g. \Name{John {Smith Jones}} similarly
% % if the name has a "von" part, e.g \Name{Jane {de Winter}}.
% % If the first letter in the forenames is a diacritic
% % enclose the diacritic in braces, e.g. \Name{{\'E}louise Smith}

% % Two authors with the same address
% % \coltauthor{\Name{Author Name1} \Email{abc@sample.com}\and
% %  \Name{Author Name2} \Email{xyz@sample.com}\\
% %  \addr Address}

% % Three or more authors with the same address:
% % \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
% %  \Name{Author Name2} \Email{an2@sample.com}\\
% %  \Name{Author Name3} \Email{an3@sample.com}\\
% %  \addr Address}

% % Authors with different addresses:
% \coltauthor{%
%  \Name{Anastasis Kratsios} \Email{kratsioa@mcmaster.ca}\\
%  \addr Address 1
%  \AND
%  \Name{Author Name2} \Email{xyz@sample.com}\\
%  \addr Address 2%
%  % \author{Anastasis Kratsios, Marc T. Law, Haitz Sáez de Oc\`{a}riz Borde, and Takashi Furuya}
% }

==> Bookkeeping/0_packages.tex <==
%%%%%%%%%%%%%%
%% Packages %%
%%%%%%%%%%%%%%
\usepackage{float}\usepackage{colortbl}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{placeins}
\usepackage{xparse}
\usepackage{color}
\usepackage{comment}
\usepackage{natbib}

\usepackage{hyperref} 
    \hypersetup{
    	colorlinks = true,
    	linkcolor = blue,
    	anchorcolor = blue,
    	citecolor = blue,
    	filecolor = blue,
    	urlcolor = blue
    }

% Fonts and such
\usepackage{accents}
\def\baselinestretch{1}
% \renewcommand{\complement}{^c}
% \newcommand{\complement}{^c}
 \DeclareMathOperator{\deb}{deb}
 \DeclareMathOperator{\conv}{conv}

% Graphics and Figures
\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}

% TABLE Formatting
% \usepackage{tablefootnote}
\usepackage{adjustbox}
\usepackage{booktabs}
\raggedbottom
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\setlength\heavyrulewidth{0.3ex}
\renewcommand{\arraystretch}{1.25}
\usepackage{lscape}








%%% COLOURs and Commenting

%
%
%
%
%
%
\usepackage{marginnote}
\usepackage{xcolor}



==> Bookkeeping/Pfaff/pfaff.tex <==
\subsection{Quantitative Estimates via Pfaffian Nonlinearities}
\label{s:Intro__ss:Pfaff}

Accordingly, we introduce the concept of Pfaffian neural networks (PNNs), an abstraction encompassing most practical architectures, except for those appearing in the super-expressive literature, as discussed previously in Section~\ref{subsec:Properties of Pfaffians}. This framework allows us to show that, although neural networks are highly nonlinear objects, their Pfaffian complexity grows in a controlled and predictable manner with depth and with the degrees of the activation functions. Additionally, in Section~\ref{sec:Transformer Blocks are Pfaffian}, we focus on establishing that the Transformer blocks underlying most modern LLMs are Pfaffian and satisfy analogous quantitative properties.


\AK{I'd like to distinguish between (trainable) Pfaffian layers, the $F_k$ below, sets of these (which in a sense are families of Pfaffian layers which generate families of Pfaffian networsk; i.e. since we view things as being trainable), and Pfaffian networks.  }
\greggy{@Annie: Can you give an example of the distinction you mean? In the setup below, all layers are assumed to be trainable, but the parameters could appear trivially in any particular layer.} \SB{Yeah, I'm not sure I get what you mean either actually}

\SB{I propose to consistently capitalize Pfaffian to honor the good old Pfaff.}

\SB{Is there a reason why we switched from $(x,\theta)$ to $(\bar{x}, \bar{\theta})$ below?}

\begin{Def}[Pfaffian Neural Networks and Pfaffian Layers]
\label{def:PfaffLayer}
Fix $n\in \mathbb{N}_+$.
% Let $n,m\in \mathbb{N}_+$ be given.  
A family $\mathcal{F}$ of Pfaffian functions is called a family of \textit{Pfaffian layers} if: for each $m\in \mathbb{N}_+$ there is a function $F:U\to \mathbb{R}^m$ defined on some non-empty domain $U\subseteq \mathbb{R}^n$ and given by
    \begin{align}
    \label{eq:PNN}
        F(\bar{x}, \bar{\theta})\eqdef \bigcirc_{k=0}^L F_k(\bar{x}_k,\bar{\theta})
    \end{align}
    % \Bum{\bigcirc_{k=0}^L F_k(\bar{x}_i,\bar{\theta}) to \bigcirc_{k=0}^L F_k(\bar{x}_k,\bar{\theta})}
    \AK{notation $\bar{\theta}_k$}[.]
    % \Bum{\bar{x} -> \bar{x}_k}
    where $F_k(\bar{x}_k,\bar{\theta})=(g_{k,1}(\bar{x}_k,\bar{\theta}),\ldots, g_{k,n_k}(\bar{x}_k,\bar{\theta}))$ for which 
    \[g_{k,i}(\bar{x}_k, \bar{\theta})=Q_{k,i}(\bar{x}_k, \bar{\theta}, f^k_1(\bar{x}_k,\bar{\theta}), \ldots, f^k_{q_k}(\bar{x}_k, \bar{\theta}))\]
         belongs to 
         $\mathcal{F}$
         and is of format $(q_k, D_k, d_{k,i})$ over a fixed Pfaffian chain $f^k_1(\bar{x}_k,\bar{\theta}), \ldots, f^k_{q_k}(\bar{x}_k, \bar{\theta})$ (in particular, it is Pfaffian in the variables $\bar{x}$ \emph{and} $\bar{\theta}$)\footnote{Note that, by assumption, $|\bar{x}_k|=n_{k-1}$ for $k\geq 2$. For $k=0$, we assume that $\bar{x}_0=\bar{x}$ and $F_0(\bar{x})=\bar{x}$. We also implicitly assume that their domains of definition are such that composition makes sense.\SB{I don't think $n_k$ was introduced at this point. And what is the meaning of the notation $|\cdot|$ in this context?}}. \SB{Note that we haven't introduced Pfaffian chains at this point}
\hfill\\
The function $F$ in~\eqref{eq:PNN} is referred to as a $\mathcal{F}$-\textit{Pfaffian neural network} ($\mathcal{F}$-PNN) generated by the layers $\mathcal{F}$, and $\bar{\theta}$ is referred to as its \textit{trainable parameter} vector.  
We suppress the notation $\mathcal{F}$-PNN in favor of PNN, when contextually clear.
\end{Def}

The indices $1\leq k \leq L$ may be considered as corresponding to ``layers'' of the network, and each $g_{k,i}$ can be thought of as a computation node in the layer $k$. We assume a high degree of symmetry across each layer for simplicity. Although this architecture is not strictly necessary, it is convenient for inductive arguments on the bounds on the format of such networks. The tuple $\bar{\theta}\in \reals^p$ will be considered a tuple of trainable parameters. We consider a fixed tuple of parameters across all layers, but one may assume that only a sub-tuple of $\bar{\theta}$ appears in each layer component $g_{k,i}$.

\begin{rmk}
    Observe that, for a node computation $g_{k,i}$, it is perfectly acceptable for the format to be of the form $(q,D,0)$, which implies that $g_{k,i}$ is \emph{constant}, and cannot be considered as a trainable parameter. However, having such a node is equivalent to shrinking the size of the layer and considering the output as a fixed (non-trainable) parameter in successive layers; in particular, constant nodes at worst decrease the Pfaffian complexity of the final computation. For this reason, we will assume throughout this paper that each $d_{k,i}\geq 1$. In other words, we allow constant nodes so long as their outputs are trainable. 
\end{rmk}

\begin{notation*}
    For a PNN $F:\reals^n\rightarrow \reals^m$ as above with $\bar{\theta}\in \reals^p$, we will say that the function is summarized by the nested tuple $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. 
\end{notation*}

% \Bum{$F_{0,i}(\bar{x},\bar{\theta})$ -> $F_{k,i}(\bar{x},\bar{\theta})$}
For an intermediate layer $1\leq k \leq L$, let $F_{k,i}(\bar{x},\bar{\theta})$ be the partial computation up to layer $k$ and in node $1\leq i \leq n_k$. The partial computation is described recursively:
\begin{enumerate}
    \item $F_{0,i}(\bar{x})=x_i$ for $1\leq i \leq n_0$,
    \item if $1\leq k\leq L$ and $1\leq i \leq n_k$, then at node $\gamma^k_i\in V_k$ we compute
        \[F_{k,i}(\bar{x}, \bar{\theta})=g_{k,i}\left(F_{k-1,1}(\bar{x},\bar{\theta}), \ldots, F_{k-1,n_{k-1}}(\bar{x},\bar{\theta}), \bar{\theta}\right).\]
\end{enumerate}
\newpage



\newpage


\subsection{Bounded Constants Under Pfaffian-Smoothness}
The above results proved that the VC and pseudo-dimensions of any definable neural network are finite, globally over their \textbf{unbounded} parameter space.  Thus, they must learn to classify and regress at the Monte Carlo rate of $\mathcal{O}(\sqrt{\log(\delta)}/\sqrt{N})$ with probability at least $1-\delta$.  

However, these results give no quantitative estimate of that pseudo-dimension at that level of generality.  The next result shows that it is explicitly estimable, still with unbounded parameter spaces and thus still working directly in the function space, under the natural notion of smoothness in the definable context; namely, Pfaffianity.  


\begin{thm}[Bounding The Pseudo-Dimension of Pfaffian Neural Networks]
\label{thrm:PNNs}
    Suppose that a PNN $F(\bar{x},\bar{y})$ is summarized by $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. Let 
    \[\calF=\{F(\bar{x},\bar{\theta}):\bar{\theta}\in \reals^p\}.\]
    Then the pseudo-dimension of $\mathcal{F}$ is bounded above by
    \begin{align*}
        \pdim(\calF) \leq 
        16p & + pq(pq-1) 
        \\
        & + p\left[\log_2(d)
        \log_2(p(D+d-1)+1)
        \right.
        \\
        & +
        \left.
        q\log_2((p+1))+q\log_2(p(D+d-1)+1)\right]
    ,
    \end{align*}
    where, 
    \begin{align*}
        q&\leq \sum_{l=1}^L q_l,\\
        D&\leq D_1+ \sum_{l=2}^L\left((D_l+1)\prod_{t=1}^{l-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}\right)-L+1, \\
        d&\leq d_{k,i}\prod_{l=1}^{L-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}.
    \end{align*}
\end{thm}

\Bum{Note that $\log$ of a product is a sum: $\log_2(ab)=\log_2 a+\log_2 b$. This requires correction to the following:
\[
	p\big[\log_2(d)\log_2(p(D+d-1)+1)+\cdots\big].
\]
After:
Starting from the manuscript's bound
\[
	B\le 2^{\frac{pq(pq-1)}{2}} d^p[p(D+d-1)+1]^p[(p+1)(p(D+d-1)+1)]^{pq},
\]
Lemma~\ref{KM-theorem} gives $\pdim(\calF)\le 16p+2\log_2 B$, hence
\begin{align*}
	\pdim(\calF) \le 16p + pq(pq-1)
	+ 2p\log_2 d
	+ 2p\log_2\big(p(D+d-1)+1\big) \\
	+ 2pq\log_2(p+1)
	+ 2pq\log_2\big(p(D+d-1)+1\big).
\end{align*}
}

\Bum{Separate from the $\log$ issue, it also defines $D$ and $d$ with incorrect indices, which affects the quantitative pseudo-dimension bound. Currently, at the end of the theorem, $D$ and $d$ are bounded using expressions of the form
	\begin{align*}
		D & \le D_1+\sum_{l=2}^L\Big((D_l+1)\prod_{t=1}^{l-1}\max_{1\le j_l\le n_l}\{d_{i,j_l}\}\Big)-L+1, \\
		d & \le d_{k,i}\prod_{l=1}^{L-1}\max_{1\le j_l\le n_l}\{d_{i,j_l}\}.
	\end{align*}
	Please replace the layer-max typos by the intended layerwise maxima and fix the output-layer index, e.g.,
	\begin{align*}
		D & \le D_1+\sum_{l=2}^L\Big((D_l+1)\prod_{t=1}^{l-1}\max_{1\le j_t\le n_t}\{d_{t,j_t}\}\Big)-L+1, \\
		d & \le d_{L,i}\prod_{l=1}^{L-1}\max_{1\le j_l\le n_l}\{d_{l,j_l}\}.
	\end{align*}
}

\paragraph{The Quantitative Agnostic PAC-Learning Bound}
Having established our main technical engine in Theorem~\ref{thrm:PNNs}, we are prepared to obtain our main quantitative agnostic PAC-learning bound for Pfaffian neural networks.




\subsubsection{Generalization via covering}
\SB{Another route is to do what they do in \cite[Section 14]{petersen2024mathematical}}

\AK{These bounds are bad, as they explode when the parameter space becomes unbounded.  This is not the case via our argument (we should make this distinction); TLDR ours work in the function space (good) theirs in the parameter space (bad) and translate to the function space via the NN-realization map.}

\SB{I thought about it, and we should be careful about ``strawmanning'' the result in \cite{petersen2024mathematical}. The thing is that there are better generalization bounds now available in the literature, even for holomorphic functions. See \cite{reinhardt2024statistical} and my recent review paper \cite[Section~2]{brugiapaglia2026short}. Essentially, it is possible to show Monte Carlo rate type bounds ($O(n^{-1/2}$ where $n$ is the data) for holomorphic operators with subgaussian random noise using "covering number"-type arguments (sharper than those used in \cite{petersen2024mathematical}). The techniques based on practical existence theory achieve instead faster (e.g., exponential) rates, but you need either zero noise or noise whose magnitude goes to zero with respect to the data $n$.}
\AK{interesting, we should chat :)
\hfill\\
Still, I think the bounds we have apply to heavy tailed distributions also; no since they're combinatorial and don't assume sub-Gaussian. (let's check).  Also, ours are also $\mathcal{O}(1/\sqrt{n})$ :D I think subtely will be on constants.
}

\SB{Yes, let's chat about it. But keep in mind that the generalization bounds in \cite{petersen2024mathematical} show that the expected squared error is $O(n^{-1/2})$. That means that the actual rate for the root of the expected square error (which is ``morally'' a standard $L^2$ error) is slower than MC, i.e., $O(n^{-1/4})$. The stuff in \cite{reinhardt2024statistical} actually leads to a MC rate.}








\subsection{Proof of Statistical Guarantees for Pfaffian Neural Networks}
\label{s:Proofs__ss:Stats___sss:Pfaff}


\paragraph{Properties of Pfaffian Functions}
\label{subsec:Properties of Pfaffians}

A fundamental result of Khovanskii bounds the number of zeros of a Pfaffian system only in terms of its format: 

\begin{lemma}[\cite{Khovanskii_Fewnomials},\cite{GabrielovVorobjov_NoetherianPfaffianComplexity_2004}]\label{khovanskii_theorem}
Consider a system of equations 
\[
f_1 = \cdots = f_n = 0,
\]
where $f_i$, $1 \le i \le n$, are Pfaffian functions in a domain $U \subset \mathbb{R}^n$, over a common Pfaffian chain of format $(q, D,d_i)$, respectively. Then the number of non-degenerate solutions of this system does not exceed
\[
\mathcal{M}(n,q,D,d_1,\ldots,d_n)  \eqdef 
2^{\frac{q(q-1)}{2}} d_1 \cdots d_n \, \big( \min\{n,q\}D + d_1 + \cdots + d_n - n + 1 \big)^q.
\]
\end{lemma}

\begin{lem}\label{pfaf-deriv-format}
    Suppose that 
    $%$\[
            g(\bar{x}) 
        = 
            Q(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}))
    $%\]
    is Pfaffian of format $(q,D,d)$ on a domain $U$. Let $x_i\in \bar{x}$. Then $\frac{\partial g}{\partial x_i}$ is also Pfaffian on $U$ of format at most $(q, D, D+d-1)$.
\end{lem}

\begin{proof}
    Let $\bar{x} = (x_1,\ldots, x_n)$ and $Q(\bar{x}, y_1,\ldots, y_q)$ be as in the statement of the lemma. 
    Observe that, for any $x_i\in \bar{x}$,  
    \begin{align*}
        \frac{\partial g(\bar{x})}{\partial x_i}&=\frac{\partial Q(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}))}{\partial x_i}\\
        &=\frac{dQ}{dx_i}(\bar{x},f_1(\bar{x}), \ldots, f_q(\bar{x})) + \sum_{j=1}^q \frac{\partial Q}{\partial y_j}(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}))\frac{\partial f_j(\bar{x})}{\partial x_i},
    \end{align*}
which is a polynomial of at most $\max\{d-1, D+d-1\}\leq D+d-1$ in the variables $\bar{x}$ and $f_1(\bar{x}), \ldots, f_q(\bar{x})$, since the first term has degree at most $d-1$ and the product term on the right has degree at most $(d-1) + D$ (degrees add under multiplication). So, by definition, $\frac{\partial g}{\partial x_i}$ is Pfaffian on $U$ over the chain $ f_1(\bar{x}), \ldots, f_q(\bar{x})$ of format at most $(q,D,D+d-1)$. 
\Bum{Consider the degenerate case $D=d=0$. For example, if $g(x)\equiv c$, then $g$ is Pfaffian of format $(0,0,0)$ over the empty chain, but $\frac{d}{dx}g(x)=0$ should still have a valid nonnegative output degree, whereas the current bound gives $D+d-1=-1$. The proof has the same problem when it treats the derivative degree as bounded by $d-1$ and $D+d-1$ in this constant case. A safe correction would be: $\frac{\partial g}{\partial x_i}$ is Pfaffian on $U$ of format at most $(q,D,\max\{0,D+d-1\})$. Equivalently, one may impose an explicit hypothesis excluding the degenerate case $D=d=0$.}
\end{proof}


\begin{cor}
Suppose that \[g(\bar{x}) = Q(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}))\] is Pfaffian of format $(q,D,d)$ on a domain $U$. Then the extended sequence
\[
(f_1(\bar{x}), \ldots, f_q(\bar{x}), g(\bar{x}))
\]
is a Pfaffian chain on $U$ of length $q+1$ and degree at most $D+d-1$.
\end{cor}

\begin{proof}
By Lemma~\ref{pfaf-deriv-format}, $\partial g / \partial x_i$ can be expressed as a polynomial in $(\bar{x}, f_1, \dots, f_q)$ of degree at most $D+d-1$.  
Thus, appending $g$ to the original chain satisfies the Pfaffian chain definition, giving a (longer) chain of length $q+1$ and the maximum degree of derivatives in the chain becomes at most $D+d-1$. The triplet format is thus $(q+1,D+d-1,d)$, since the function degree itself does not change.
\end{proof}
\Bum{Check when $d=0$. For example, starting from the chain $(e^x)$ of degree $D=1$ and taking $g\equiv 0$, the extended chain $(e^x,0)$ still has chain degree $1$. Replace the conclusion with a degree bound of $\max\{D,D+d-1\}$, or explicitly assume $d\ge 1$. Note that other parts allow $d=0$, so I think the former would be reasonable.}

\begin{lem}\label{pfaff-product-format}
    Suppose 
    \[f(\bar{x})\in \reals[\bar{x}, f_1(\bar{x}),\ldots, f_{q_f}(\bar{x})]\]
    and 
    \[g(\bar{x})\in \reals[\bar{x}, g_1(\bar{x}),\ldots, g_{q_g}(\bar{x})]\]
    are Pfaffian of format $(q_f,D_f,d_f)$ and $(q_g, D_g, d_g)$, respectively over the chains $f_1(\bar{x}),\ldots, f_{q_f}(\bar{x})$ and $g_1(\bar{x}),\ldots, g_{q_g}(\bar{x})$ on a common domain $U$. Then $f(\bar{x})g(\bar{x})$ is Pfaffian on $U$ of format at most $(q_f+q_g, \max\{D_f,D_g\}, d_f+d_g)$. 
\end{lem}

\begin{proof}
    The concatenation of the chains $f_1(\bar{x}),\ldots, f_{q_f}(\bar{x}), g_1(\bar{x}), \ldots, g_{q_g}(\bar{x})$ is a Pfaffian chain on $U$ of length $q_f+q_g$ (worst-case upper bound argument, without trying to reduce the number of functions or account for any overlap between the chains) and degree $\max\{D_f, D_g\}$ (upper bound treating the chains as disjoint). Let $Q_f(\bar{x}, y_1,\ldots y_{q_f})$ be of degree $d_f$ and $Q_g(\bar{x}, z_1,\ldots, z_{q_g})$ be of degree $d_g$ be such that 
    \begin{align*}
        f(\bar{x})&=Q_f(\bar{x}, f_1(\bar{x}),\ldots, f_{q_f}(\bar{x}))\\
        g(\bar{x})&=Q_g(\bar{x}, g_1(\bar{x}),\ldots, g_{q_g}(\bar{x})).
    \end{align*}
    Then $Q_f(\bar{x}, \bar{y})Q_g(\bar{x},\bar{z})$ has degree at most $d_f+d_g$.
\end{proof}

\begin{lem}\label{pfaff-sum-format}
    Suppose 
    \[f(\bar{x})\in \reals[\bar{x}, f_1(\bar{x}),\ldots, f_{q_f}(\bar{x})]\]
    and 
    \[g(\bar{x})\in \reals[\bar{x}, g_1(\bar{x}),\ldots, g_{q_g}(\bar{x})]\]
    are Pfaffian of format $(q_f,D_f,d_f)$ and $(q_g, D_g, d_g)$, respectively, on a common domain $U$. Then $f(\bar{x})+g(\bar{x})$ is Pfaffian on $U$ of format at most $(q_f+q_g, \max\{D_f,D_g\}, \max\{d_f,d_g\})$.
\end{lem}

\begin{proof}
    As in Lemma~\ref{pfaff-product-format}, we may concatenate the chains to obtain a Pfaffian chain of length $q_f+q_g$ and degree $\max\{D_f,D_g\}$ (a worst-case upper bound, ignoring possible overlaps). Concatenation is necessary here (just as in the product case), since $f$ and $g$ may be defined with respect to different chains, and the Pfaffian definition requires that the sum be expressed as a polynomial in a single common chain. Since addition cannot increase polynomial degree, the total degree of the sum is determined by the highest-degree monomial appearing in either $Q_f$ or $Q_g$. Hence the degree of $Q_f+Q_g$ is at most $\max\{d_f,d_g\}$.
\end{proof}

\begin{lem}
    Suppose $f(\bar{x})$ and $g(\bar{x})$ are Pfaffian functions of format $(q,D,d_f)$ and $(q,D,d_g)$, respectively, on a domain $U$, i.e.\ both are defined with respect to the same Pfaffian chain of length $q$ and degree $D$. Then: the product $f(\bar{x})g(\bar{x})$ is Pfaffian on $U$ of format $(q,D,d_f+d_g)$, and the sum $f(\bar{x})+g(\bar{x})$ is Pfaffian on $U$ of format $(q,D,\max\{d_f,d_g\})$.
\end{lem}

\begin{proof}
    Since $f$ and $g$ are defined with respect to the same chain, we do not need to enlarge the chain (unlike in Lemmas~\ref{pfaff-product-format} and \ref{pfaff-sum-format}). Thus the parameters $q$ (length) and $D$ (degree of the chain) are preserved. The product polynomial has degree at most $d_f+d_g$, while the sum has degree at most $\max\{d_f,d_g\}$.
\end{proof}

\begin{eg}
    Pfaffianity as a property is preserved under composition, but the chain that realizes it is not necessarily preserved. Consider the exponential function $f(x) = e^x.$ This forms a Pfaffian chain of length $q=1$ and degree $D=1$ on $\mathbb{R}$, since $f'(x) = e^x = f(x),$ which is a polynomial of degree 1 in the chain variable $f(x)$. Hence $f$ is Pfaffian of format $(1,1,1)$. Now consider the composition $g(x) = e^{e^x}.$ This function is also Pfaffian, but it cannot be expressed over the original chain $(e^x)$ alone. Instead, we form a new chain $f_1(x) = e^x, f_2(x) = e^{e^x},$ of length $q=2$. Its derivatives are $f_1'(x) = f_1(x), f_2'(x) = f_2(x) f_1(x) = e^{e^x} e^x,$ which are polynomials of degree at most $2$ in the variables $(x, f_1, f_2)$. Thus $g$ is Pfaffian of format $(2,2,1)$. In other words, the property of being Pfaffian is preserved by composition, but the chain that realizes the Pfaffian representation must often be \textit{extended}.
\end{eg}


\begin{lem}\label{pfaff-chain-composition}
Let $\calF = (f_1(\bar{x}), \dots, f_q(\bar{x}))$ be a Pfaffian chain of degree $D$ on a domain $U_\calF$. For $i=1,\dots,n$, let  
$h_i(\bar{x}) = R_i(\bar{x}, f_1(\bar{x}), \dots, f_q(\bar{x}))$  
be Pfaffian functions of format $(q,D,d_i)$ over $\calF$. Let $\calG = (g_1(\bar{y}), \dots, g_{q'}(\bar{y}))$ be a Pfaffian chain of degree $D'$ on a domain $U_\calG$, and assume that  
$(h_1(\bar{x}), \dots, h_n(\bar{x})) \in U_\calG$ for all $\bar{x} \in U_\calF$. Define $s_j(\bar{x}) = g_j(h_1(\bar{x}), \dots, h_n(\bar{x}))$ for $j=1,\dots,q'$. Then the concatenated chain  
\[
(f_1(\bar{x}), \dots, f_q(\bar{x}), s_1(\bar{x}), \dots, s_{q'}(\bar{x}))
\]
is Pfaffian on $U_\calF$, of length $q + q'$ and degree at most  
$D + (D' + 1)\max_i\{d_i\} - 1$.
\end{lem}

\begin{proof}
Let $\{P_{i,j}: 1 \le i \le q', \, 1 \le j \le n\}$ be the polynomials of degree at most $D'$ witnessing the Pfaffianity of $\calG$. Consider the sequence $f_1, \dots, f_q, s_1, \dots, s_{q'}$. The first $q$ functions form a Pfaffian chain of degree $D$ by assumption. For each $i = 1, \dots, q'$ and variable $x_k$, the chain rule gives
\[
\frac{\partial s_i}{\partial x_k} = \sum_{j=1}^n P_{i,j}(h_1, \dots, h_n, s_1, \dots, s_i) \frac{\partial h_j}{\partial x_k}.
\]

Each $h_j$ is polynomial in $(\bar{x}, f_1, \dots, f_q)$ of degree $\le d_j$. Substituting $h_1, \dots, h_n$ into $P_{i,j}$ gives a polynomial in $(\bar{x}, f_1, \dots, f_q, s_1, \dots, s_i)$. The degree of this composition is obtained by multiplying the degree of $P_{i,j}$ (which is $\le D'$) by the maximum degree of the $h_j$’s (which is $\max_j {d_j}$), giving degree $\le D' \max_j{d_j}$.

Next, by Lemma~\ref{pfaf-deriv-format}, $\partial h_j / \partial x_k$ is polynomial of degree $\le D + d_j - 1$. Each term in the sum $\sum_{j=1}^n P_{i,j}(h_1, \dots, h_n, s_1, \dots, s_i) , \partial h_j / \partial x_k$ is a product of two polynomials, so the degrees add. Hence, the degree of each term is at most $D' \max_j {d_j} + (D + \max_j {d_j} - 1) = D + (D' + 1)\max_j {d_j} - 1$.

Since all derivatives of the first $q$ functions have degree $\le D$, this bound is always at least $D$. Therefore, the concatenated sequence $f_1, \dots, f_q, s_1, \dots, s_{q'}$ forms a Pfaffian chain of length $q + q'$ and degree at most $D + (D' + 1)\max_i {d_i} - 1$.
\end{proof}

\Bum{For example, if every $h_i$ is constant, then substituting the $h_i$ into a degree-$D'$ polynomial $P_{i,j}$ still leaves a polynomial of degree up to $D'$ in the chain variables $s_1,\dots,s_i$, whereas the manuscript's bound gives
	\begin{align*}
		D'\max_i d_i = 0.
	\end{align*}
	Likewise, the chain-degree bound
	\begin{align*}
		D+(D'+1)\max_i d_i-1
	\end{align*}
	can even drop below $D$ or become negative when $\max_i d_i=0$, contradicting the proof's sentence that this bound is always at least $D$. I found that the later PNN section remarks that node degrees are assumed to satisfy $d_{k,i}\ge 1$, which avoids this issue in that specific application, but Lemmata \ref{pfaff-chain-composition}, \ref{pfaff-composition-function}, and \ref{pfaff-comp-format-bound} are currently stated without that restriction. Please assume explicitly that every inner format degree satisfies $d_i\ge 1$.}


\begin{lem}\label{pfaff-composition-function}
Let $\alpha(\bar{y}) = Q(\bar{y}, g_1(\bar{y}), \dots, g_{q'}(\bar{y}))$ be Pfaffian of format $(q',D',d')$ over the chain $\calG$ from Lemma~\ref{pfaff-chain-composition}. Define  
$w(\bar{x}) = \alpha(h_1(\bar{x}), \dots, h_n(\bar{x}))$,  
with $h_i$ and $s_j$ as in Lemma~\ref{pfaff-chain-composition}. Then $w(\bar{x})$ is Pfaffian over the concatenated chain  
\[
(f_1(\bar{x}), \dots, f_q(\bar{x}), s_1(\bar{x}), \dots, s_{q'}(\bar{x}))
,
\]
with format at most $(q+q', D+(D'+1)\max\{d_j\}-1, d'\max\{d_j\})$ on the domain $U_{\calF}$.
\end{lem}

\begin{proof}
\begin{align*}
        w(\bar{x}) 
        &= \alpha(h_1(\bar{x}), \ldots, h_n(\bar{x}))\\
        &= Q(h_1(\bar{x}), \ldots, h_n(\bar{x}), s_1(\bar{x}), \ldots, s_{q'}(\bar{x}))\\
        &= Q(R_1(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})), \ldots, 
              R_n(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})), 
              s_1(\bar{x}), \ldots, s_{q'}(\bar{x})).
\end{align*}
Each $h_i$ is a polynomial of degree $\le d_i$ in $(\bar x,f_1,\dots,f_q)$ by assumption. Since $Q$ has total degree $\le d'$ in its arguments, any monomial of $Q$ after substitution becomes
\[
\prod_i R_i^{a_i}\cdot \prod_j s_j^{b_j},\qquad \sum_i a_i+\sum_j b_j\le d'.
\]
Its degree in $(\bar x,f_1,\dots,f_q,s_1,\dots,s_{q'})$ is at most 
\begin{align*}
\sum_i a_i d_i + \sum_j b_j 
&\le \sum_i a_i \max_i d_i + \sum_j b_j \\
&\le \left(\sum_i a_i\right) \max_i d_i + \left(\sum_j b_j\right) \max_i d_i \\
&= \left(\sum_i a_i + \sum_j b_j \right) \max_i d_i \\
&\le d' \max_i d_i.
\end{align*} 
Hence $w$ has degree at most $d'\max_i d_i$. The bounds on chain length and chain degree follow directly from Lemma~\ref{pfaff-chain-composition}.
\end{proof}



\begin{lem}\label{pfaff-comp-format-bound}
 Let $\calF=\{f_1(\bar{x}),\ldots, f_q(\bar{x})\}$
 be Pfaffian of degree $D$ over on a domain $U_{\calF}$, and, for each $1\leq i \leq n$, let 
 \[h_i(\bar{x})=R_i(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}))\]
 be Pfaffian of format $(q,D, d_i)$ over $\calF$. Let 
 \[\calG =\{g_1(\bar{y}), \ldots, g_{q'}(\bar{y})\}\]
 be Pfaffian of degree $D'$ on a domain $U_{\calG}$, such that $\bar{y}=(y_1,\ldots, y_n)$, and let 
 \[\alpha(\bar{y})=Q(\bar{y},g_1(\bar{y}), \ldots, g_{q'}(\bar{y}))\]
 be Pfaffian of format $(q', D', d')$ over $\calG$. Assume that for each $\bar{x}\in U_{\calF}$, $(h_1(\bar{x}),\ldots,h_n(\bar{x}))\in U_{\calG}$. Consider the compositions 
 \[w(\bar{x})=\alpha(h_1(\bar{x}), \ldots, h_n(\bar{x}))\]
 and, for $1\leq j \leq q'$, 
 \[s_j(\bar{x})=g_j(h_1(\bar{x}), \ldots, h_n(\bar{x})).\]
 Then the chain 
 $%$\[
    f_1(\bar{x}), \ldots, f_q(\bar{x}),s_1(\bar{x}), \ldots, s_{q'}(\bar{x}) 
 $%$\] 
 is Pfaffian of degree $D+(D' + 1)\max\{d_j\}-1$, and $w(\bar{x})$ is Pfaffian over the chain with format at most $(q+q', D+(D'+1)\max\{d_j\}-1, d'\max\{d_j\})$ on the domain $U_{\calF}$.
\end{lem}

\begin{proof}
    Let $\{P_{i,j}:1\leq i \leq q', 1\leq j\leq n\}$ be polynomials of degree at most $D'$ witnessing the Pfaffianity of $\calG$. First, we show that 
    \[f_1(\bar{x}), \ldots, f_q(\bar{x}), s_1(\bar{x}), \ldots, s_{q'}(\bar{x})\]
    is a Pfaffian chain. The first $q$-many functions form a Pfaffian chain of degree $D$ by assumption. For $1\leq i \leq q'$ and $1\leq j,k\leq n$, we have
    \begin{align*}
        \deriv{s_i(\bar{x})}{x_k}&=\deriv{g_i(h_1(\bar{x}), \ldots ,h_n(\bar{x}))}{x_k}\\
        &=\sum_{j=1}^n P_{i,j}(h_1(\bar{x}),\ldots, h_n(\bar{x}), s_1(\bar{x}), \ldots, s_i(\bar{x}))\deriv{h_j(\bar{x})}{x_k}.
    \end{align*}
    By assumption, each $h_j(\bar{x})$ is polynomial in the variables $\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})$ of degree at most $d_j$, and so 
    \[P_{i,j}(h_1(\bar{x}), \ldots, h_n(\bar{x}), s_1(\bar{x}), \ldots, s_{i}(\bar{x}))\]
    is polynomial in the variables \\ 
    $\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}), s_1(\bar{x}),\ldots, s_i(\bar{x})$ of degree at most $D'\max_{1\leq j \leq n}\{d_j\}$. 
    By Lemma \ref{pfaf-deriv-format}, $\deriv{h_j}{x_k}$ is polynomial in the variables $\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})$ of degree at most $D+d_j-1$. Thus, each term is polynomial in the variables $\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x}), s_1(\bar{x}), \ldots, s_{q'}(\bar{x})$ with degree at most $D+(D'+1)\max_{1\leq j \leq n}\{d_j\}-1$. In other words, \\
    $f_1(\bar{x}), \ldots, f_q(\bar{x}), s_1(\bar{x}), \ldots, s_{q'}(\bar{x})$ is a Pfaffian chain of length $q+q'$ and degree at most $D+(D'+1)\max_{1\leq j \leq n}\{d_j\}-1.$
    Now, 
    \begin{align*}
        w(x)&=\alpha(h_1(\bar{x}), \ldots, h_n(\bar{x}))\\
        &=Q(h_1(\bar{x}),
        \ldots, h_n(\bar{x}),s_1(\bar{x}), \ldots, s_{q'}(\bar{x}))\\
        &=Q(R_1(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})),\ldots,R_n(\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})),s_1(\bar{x}),\ldots, s_{q'}(\bar{x}))
    \end{align*}
    is clearly polynomial in the variables $\bar{x}, f_1(\bar{x}),\ldots, f_q(\bar{x}), s_1(\bar{x}), \ldots s_{q'}(\bar{x})$ with degree at most $d'\max_{1\leq j\leq n}\{d_j\}$.
\end{proof}

% Solved
%\Bum{Check Typos. Before: \\
%	$\deriv{h_j}{x_k}$ is polynomial in $\bar{x}, f_1(\bar{x}), \ldots, f_1(\bar{x})$. $\dots,s_1(\bar{x}),\ldots, s_q'(\bar{x})$. \\
%	After: \\
%	$\deriv{h_j}{x_k}$ is polynomial in $\bar{x}, f_1(\bar{x}), \ldots, f_q(\bar{x})$. $\dots,s_1(\bar{x}),\ldots, s_{q'}(\bar{x})$.
%}

\begin{cor}\label{cor:pfaff-substitution}
    Let $\calF=(f_1(\bar{x},\bar{y}),\ldots, f_q(\bar{x},\bar{y}))$ be a Pfaffian chain of length $q$ and degree $D$ in the variables $(\bar{x},\bar{y})=(x_1,\ldots, x_k, y_1,\ldots, y_l)$ and suppose $g(\bar{x},\bar{y})$ is Pfaffian over $\calF$ of format at most $(q,D,d)$. Let $\bar{\alpha}_1, \ldots \bar{\alpha}_n\in \reals^k$. Then 
    \[\hat\calF=(f_i(\bar{\alpha}_j,\bar{y}):1\leq i \leq q, 1\leq j \leq n)\]
    form a Pfaffian chain of length $nq$ and degree at most $D$.
\end{cor}

\begin{proof}
Substituting $\bar{x} = \bar{\alpha}_j$ does not increase the degree $D$, because a polynomial in constants is still a polynomial of the same degree in the remaining variables. Concatenating the $n$ chains for $j=1,\dots,n$ increases the length to $nq$ without increasing the degree.
\end{proof}



\paragraph{Bounding the Format of Pfaffian Neural Networks}
Having established many of the key properties of Pfaffian functions required to compute the number of connected components of parametric Pfaffian functions, we are now prepared to obtain a pseudo-dimension bound.  This will be obtained by Khovanskii's theorem, however, in order to apply those results quantitatively, we need to first quantify the format of Pfaffian neural networks.


\begin{prop}\label{prop:PNN_format}
     Suppose that a PNN is summarized by $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. For each $1\leq k\leq L$ and each $1\leq i \leq n_k$, $F_{k,i}(\bar{x}, \bar{\theta})$ is Pfaffian of format at most
    \begin{align*}
       \left(\sum_{l=1}^kq_l,  \sum_{l=1}^k\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_t \leq n_t}\{d_{t,j_t}\}\right)-k, d_{k,i}\prod_{l=0}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}\right)
    \end{align*}
\end{prop}

\begin{proof}
We proceed inductively on the layer:
\greggy{Not worth fighting about, but I don't really love this formatting with all the hfill's. I think it would be nicer/more readable to use an itemize environment.} \SB{Let's fight. Itemize will intend everything on the right though... a lot of extra unnecessary white space :/}
\AK{Ya and itemize looks ugly (it gives me daymares)  KO Greggy}
\hfill\\
\textit{The Case where $k=0$:}
\hfill\\
    % \begin{itemize}
% \item 
        For $k=0$, the input layer, $F_{0,i}(\bar{x}, \bar{\theta})=x_i$ is trivially Pfaffian of format $(q_0, D_0, d_{0,i})=(0,0,1)$. 
\hfill\\
\textit{The Case where $k=1$:}
\hfill\\
% \item 
        For $k=1$, $F_{1,i}(\bar{x},\bar{\theta})=g_{1,i}(\bar{x},\bar{\theta})$, which is Pfaffian of format
        \begin{align*}
           (q_1, D_1, d_{1,i})&=(q_1+q_0,D_0+(D_1+1)\max_{1\leq j \leq n_0}\{d_{0,j}\}-1,d_{1,i}\max_{1\leq j \leq n_0}\{d_{0,j}\})\\
           &=(q_1+q_0,(D_1+1)\max_{1\leq j \leq n_0}\{d_{0,j}\}-1,d_{1,i}\max_{1\leq j \leq n_0}\{d_{0,j}\})
        \end{align*}
        by a direct application of Lemma \ref{pfaff-comp-format-bound}.
        % \greggy{In fact, this suffices as the base case, though I think $k=2$ is illustrative. We can remove it if we want to save some space. }\ocariz{I have a preference for being as illustrative as possible}
        % \greggy{@ocariz, I agree completely. I just also want to be conscious of space. Not including k=2 wouldn't make it less correct, and would save a few lines. For me, I'm fine either way. It's you people who are obsessed with size.}
\hfill\\
\textit{The Case where $k=2$:}
\hfill\\
% \item 
    For $k=2$, each function 
        \[F_{2,i}(\bar{x},\bar{\theta})=g_{2,i}(F_{1,1}(\bar{x},\bar{\theta}),\ldots, F_{1,n_1}(\bar{x}, \bar{\theta}), \bar{\theta})\]
        is Pfaffian of format at most 
        \begin{align*}
        &(q_1+q_2, D_1+(D_2+1)\max_{1\leq j\leq n_1}\{d_{1,j}\}-1, d_{2,i}\max_{1\leq j\leq n_1}\{d_{1,j}\})\\&=(q_1+q_2, (D_1+1)\max_{1\leq j_0\leq n_0}+(D_2+1)\max_{1\leq j_1\leq n_1}\{d_{1,j_1}\}-2, d_{2,i}\max_{1\leq j_1\leq n_1}\{d_{1,j_1}\})
        \end{align*}
        by a direct application of Lemma \ref{pfaff-comp-format-bound}.
\hfill\\
\textit{The General Case, i.e.\ the inductive step:}
\hfill\\
% \item 
        Suppose that for the $i$-th node of layer $k$, $F_{k,i}(\bar{x}, \bar{\theta})$ is Pfaffian with format 
        \[(q_k', D_k', d_{k,i}')= \left(\sum_{l=1}^kq_l,  \sum_{l=1}^k\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_t \leq n_t}\{d_{t,j_t}\}\right)-k, d_{k,i}\prod_{l=0}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}\right).\]
        Consider a node computation 
        \[F_{k+1,i}(\bar{x},\bar{\theta})=g_{k+1, i}(F_{k,1}(\bar{x}, \bar{\theta}),\ldots F_{k,n_k}(\bar{x},\bar{\theta}), \bar{\theta}),\]
        where $g_{k+1,i}$ is Pfaffian of format at most $(q_{k+1}, D_{k+1}, d_{k+1,i})$. By Lemma \ref{pfaff-comp-format-bound}, the composition is Pfaffian of format 
        \begin{align*}
        (q_{k+1}', D'_{k+1}, d_{k+1,i}')=\left(q_{k+1}+q_k', D_{k}'+(D_{k+1}+1)\max_{1\leq j\leq n_k}\{d'_{k,j}\}-1,d_{k+1}\max_{1\leq j\leq n_k}\{d'_{k,j}\}\right).
        \end{align*}
        Then $q_{k+1}'=q_{k+1}+\sum_{l=1}^{k}q_l=\sum_{l=1}^{k+1}q_l$ and we have
        \begin{align*}
            D'_{k+1}&=D_{k}'+(D_{k+1}+1)\max_{1\leq j\leq n_k}\{d'_{k,j}\}-1\\
            &= \sum_{l=1}^k\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_t \leq n_t}\{d_{t,j_t}\}\right)-k+(D_{k+1}+1)\max_{1\leq j\leq n_k}\left\lbrace d_{k,j}\prod_{l=1}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{l,j_l}\}\right\rbrace-1\\
            &= \sum_{l=1}^k\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_t \leq n_t}\{d_{t,j_t}\}\right)+(D_{k+1}+1)\max_{1\leq j\leq n_k}\left\lbrace d_{k,j}\prod_{l=1}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{l,j_l}\}\right\rbrace-(k+1)\\
            &\leq  \sum_{l=1}^k\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_l \leq n_l}\{d_{t,j_l}\}\right)+(D_{k+1}+1)\max_{1\leq j\leq n_k}\{d_{k,j}\}\left\lbrace \prod_{l=1}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{l,j_l}\}\right\rbrace-(k+1)\\
            &=\sum_{l=1}^{k+1}\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_l \leq n_l}\{d_{t,j_l}\}\right)-(k+1).
            \end{align*}
            Finally,
            \begin{align*}
                d_{k+1,i}'&=d_{k+1,i}\max_{1\leq j \leq n_k}\{d'_{k,j}\}\\
                &=d_{k+1,i}\max_{1\leq j \leq n_k}\left\lbrace d_{k,j}\prod_{l=1}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{l,j_l}\}\right\rbrace\\
                &\leq d_{k+1,i}\max_{1\leq j \leq n_k}\{d_{k,j}\}\prod_{l=1}^{k-1}\max_{1\leq j_l \leq n_l}\{d_{l,j_l}\}\\
                &=d_{k+1,i}\prod_{l=1}^k\max_{1\leq j_l\leq n_l}\{d_{l,j_l}\}.
            \qedhere
            \end{align*}
            % as required. 
    % \end{itemize}
\end{proof}

\Bum{Check index typos in the product and max expressions, which change the meaning of the format bound and propagate to downstream corollaries. Specifically, use the layer index in the products and maxima, e.g.,
	\[
		d_{k,i}\prod_{l=0}^{k-1}\max_{1\le j_l\le n_l}\{d_{l,j_l}\}
	\]
	with the convention $d_{0,j}=1$ on the input layer, and define $d\eqdef \max_{1\le k\le L,\ 1\le j\le n_k}\{d_{k,j}\}$. Also fix the proof-display typos so the inductive update reads $d'_{k+1,i}=d_{k+1,i}\max_{1\le j\le n_k}\{d'_{k,j}\}$ and the $k=2$ base case includes $\max_{1\le j_0\le n_0}\{d_{0,j_0}\}$. This matches the inductive step where each composition multiplies by the previous layer maximum degree.}



\begin{cor}
    Suppose that a PNN is summarized by $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. Then the output components are Pfaffian of format at most 
    \[   \left(\sum_{l=1}^L q_l, \sum_{l=1}^L\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}\right)-L, d_{k,i}\prod_{l=1}^{L-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}\right)\]
\end{cor}

\Bum{This one repeats the same index mistakes and also uses an inconsistent output-layer index. Use only the layer index inside each maximum, and fix the output-layer index, e.g.,
	\begin{align*}
		d_{\mathrm{out},i} & \le d_{L,i}\prod_{l=1}^{L-1}\max_{1\le j_l\le n_l}\{d_{l,j_l}\},                         \\
		D_{\mathrm{out}}   & \le \sum_{l=1}^L\Big((D_l+1)\prod_{t=0}^{l-1}\max_{1\le j_t\le n_t}\{d_{t,j_t}\}\Big)-L,
	\end{align*}
	with the convention $d_{0,j}=1$ on the input layer.}


\begin{rmk}[Simplification]
Consider a PNN summarized by $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. Let $\hat{x}=(\bar{x}_1,\ldots,\bar{x}_n)$ (where $\bar{x}_j$ are the variables for the $j$-th layer). Then we may concatenate the Pfaffian chains associated to each layer to get a single chain of length $q=\sum_{1\leq k\leq L}q_k$ and degree $D=\max_{1\leq k \leq L}D_k$ in the variables $(\hat{x},\bar{\theta})$. In this case, let $h_1(\hat{x},\bar{\theta}),\ldots h_{q}(\hat{x},\bar{\theta})$ be the given chain of length $q$ and degree $D$. Then each node computes a function $g_{k,i}(\bar{x}_k,\hat{x}, \bar{\theta})=Q_{k,i}(\bar{x}_k,\bar{\theta}, h_1(\hat{x},\bar{\theta}), \ldots h_q(\hat{x},\bar{\theta}))$ that is Pfaffian of format $(q, D, d_{k,i})$, where $d_{k,i}$ is the degree of $Q_{k,i}$. Note that for each node computation $g_{k,i}(\bar{x}_k,\hat{x}, \bar{\theta})$, not every variable of $\hat{x}$ actually appears in the computation. Also, $\bar{x}_k$ appears also in $\hat{x}$, but this redundancy is just for notational reasons. This gives a coarser picture, but it simplifies bounding the Pfaffianity of the circuit. 
\end{rmk}

\begin{cor}[Simplified Bound]\label{simple-bound}
Suppose that a PNN is summarized by $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. Let $q=\sum q_i$, $D=\max\{D_i\},$ and  $d=\max_{1\leq k \leq L, 1\leq j \leq n_k}\{d_{i,j}\}$. Then the output nodes are Pfaffian of format at most $(q,(D+1)(L-1)d^{L-1},d^L)$.   
\end{cor}
\begin{proof}
    The bound on the chain length and the degree of the outputs over the chain are immediate. Let us consider the degree of the chain. Substituting $D=D_i$ and $d=d_{i,j}$ for all $i,j$ gives
    \begin{align*}
         \sum_{l=1}^L\left((D_l+1)\prod_{t=0}^{l-1}\max_{1\leq j_l \leq n_l}\{d_{i,j_l}\}\right)-L&\leq \sum_{l=1}^L\left((D+1)\prod_{t=0}^{l-1}\max_{1\leq j_l \leq n_l}\{d\}\right)-L\\
        &=(D+1)\left(\sum_{l=1}^L d^{l-1}\right)-L\\
        &=(D+1)\sum_{l=1}^{L-1}d^l-L
    \end{align*}
    For $d=1$, we have 
    \begin{align*}
        (D+1)\sum_{l=1}^{L-1}d^l-L&=(D+1)(L-1)-L\\
        &<(D+1)(L-1)
    \end{align*}
    Otherwise, for $d\geq 2$, the geometric sum gives
    \begin{align*}
        (D+1)\sum_{l=1}^{L-1}d^l-L&=(D+1)\left(\frac{d^L-d}{d-1}\right)-L\\
        &<(D+1)(L-1)d^{L-1}-L\\
        &<(D+1)(L-1)d^{L-1}.
    \end{align*}
    Note that this can be sharpened by noting that $d_{0,j}=1$ for all input nodes $x_j$.   
\end{proof}

\Bum{The proof drops the leading $1$ in the geometric series and shifts indices:
	\[
		(D+1)\sum_{\ell=1}^L d^{\ell-1} \not= (D+1)\sum_{\ell=1}^{L-1} d^{\ell}.
	\]
	Before:
	\[
		(D+1)\Big(\sum_{\ell=1}^L d^{\ell-1}\Big)-L =(D+1)\sum_{\ell=1}^{L-1}d^\ell-L.
	\]
	After:
	\begin{align*}
		(D+1)\Big(\sum_{\ell=1}^L d^{\ell-1}\Big)-L = (D+1)\sum_{j=0}^{L-1}d^j-L \le (D+1)Ld^{L-1},
	\end{align*}
	since $\sum_{j=0}^{L-1} d^j\le Ld^{L-1}$ for $d\ge 1$. This suggests the simplified bound $(q,(D+1)(L-1)d^{L-1},d^L)$ should be revisited. It fails already for small $L$ unless extra restrictions are imposed.
}


\paragraph{Bounding the Pseudo-Dimension of Pfaffian Neural Networks}
With the above computations in hand, we can now bound the pseudo-dimension of Pfaffian neural networks by combining the techniques of Krzysztof Karpinski and Angus Macintyre~\cite{karpinski1997polynomial} with Askold Khovanskii's theorem~\cite{Khovanskii_Fewnomials}.

\noindent
Indeed, for $C^\infty$ functions $f_i(\bar{x},\bar{y}):\reals^{n+p}\rightarrow \reals, 1\leq i \leq s$, 
consider $\reals$ as an $L$-structure in an expansion, $L$, of the language of ordered rings together with a symbol for each $f_i$ \greggy{(we will abuse notation and identify each function with its symbol... naughty naughty!)}. For a quantifier-free $L$-formula $\phi(\bar{x},\bar{y})$ and a tuple $\bar{\theta}\in \reals^p$, write
\[\phi_{\bar{\theta}}=\{\bar{a}\in \reals^n:\reals\models \phi(\bar{a},\bar{\theta})\},\]
i.e. the set defined by $\phi(\bar{x}, \bar{\theta})$.
In \cite{karpinski1997polynomial} the authors prove the following conditional bound on the VC-dimension of the class $\calC_{\phi}=\{\phi_{\bar{\theta}}:\bar{\theta}\in\reals^p\}$

\begin{lem}[\cite{karpinski1997polynomial}, Theorem 2]\label{KM-theorem}
    Suppose that there is a number $B$ such that for any choice of $\bar{a}_1,\ldots,\bar{a}_V\in \reals^k$, any choice of $C^\infty$ functions \[\tau_1(\bar{y}), \ldots, \tau_r(\bar{y})\in \{f_i(\bar{a}_j,\bar{y}):1\leq i \leq s, 1\leq j\leq V\},\]
    (with $r\leq p$) and any $\varepsilon_1,\ldots, \varepsilon_r\in \reals$, the set 
    \[\Xi^{-1}(\varepsilon_1,\ldots, \varepsilon_r) \eqdef \{\bar{y}\in\reals^p:\tau_i(\bar{y})=\varepsilon_i, 1\leq i\leq r\}\]
    is either empty or is an $(p-r)$-dimensional $C^\infty$-submanifold of $\reals^p$ with at most $B$-many connected components. Then the VC-dimension of $\calC_\phi$ is at most 
    \[2\log_2B+(16+2\log_2s)p.\]
\end{lem}

Suppose a PNN is summarized by $((n,m,p),(q_k, D_k, d_{k,i}), 1\leq i \leq n_k, 1\leq k \leq L)$. We would like to bound the pseudo-dimension of the output nodes. Without loss of generality, let us assume that $n_L=1$, and so we will refer to the computation of the single output node as $F(\bar{x},\bar{y})=F_L(\bar{x},\bar{y})$. Write $(q,D,d)$ for the format bound derived in Proposition \ref{prop:PNN_format}. Let $|\bar{x}|=n$ and $|\bar{y}|=p$.

By a gross abuse of notation, let us again consider $\reals$ in the language of ordered rings expanded by a single function symbol $F(\bar{x},\bar{y})$. Consider the quantifier-free formula given by 
\[\phi(\bar{x},\bar{y},z)=F(\bar{x},\bar{y})-z>0.\]
For a tuple $\bar{\theta}\in \reals^{p}$, and
\[\phi_{\bar{\theta}}=\{(\bar{a},c)\in \mathbb{R}^{n+1}:\reals\models\phi(\bar{a},\bar{\theta},c)\}\]
we aim to bound the VC-dimension of the class $\calC_\phi=\{\phi_{\bar{\theta}}:\bar{\theta}\in \reals^{p}\}$.

By Lemma~\ref{KM-theorem}, it suffices to find a bound $B$ satisfying the assumptions of the theorem for the associated class of functions 
\begin{align*}
    &G:\reals^{n+p+1}\rightarrow \reals\\
    &G(\bar{x},\bar{y},z)=F(\bar{x},\bar{y})-z.
\end{align*}

Observe that $G(\bar{x},\bar{y},z)$ is also Pfaffian with format no greater than that of $F(\bar{x},\bar{y})$ (on an enlarged domain) since 
\[\deriv{G}{z}=F_L(\bar{x},\bar{y})-1.\]

\Bum{The derivative of the auxiliary function $G(\bar x,\bar y,z)=F(\bar x,\bar y)-z$ is computed incorrectly. The manuscript writes $\partial G/\partial z = F_L(\bar x,\bar y)-1$. However, because $G(\bar x,\bar y,z)=F(\bar x,\bar y)-z$, we have $\partial G/\partial z=-1$, which is a constant, hence Pfaffian. The Pfaffian-format argument still goes through, but the derivative must be corrected.}

With this in mind, we appeal to a result of Khovanskii:

\begin{lem}[\cite{Khovanskii_Fewnomials}, p. 91, Example 3]\label{Kohv-bound}
Let $f_1(\bar{y}), \ldots, f_q(\bar{y})$ 
be a Pfaffian chain of length $q$ and degree $D$ in the variables $\bar{y}=(y_1,\ldots, y_m)$. Let $Q_{i}(\bar{y})$, $1\leq i \leq r$ be Pfaffian over the chain of format $(q, D, d_i)$, respectively. Then the number of connected components of the $(m-r)$-dimensional submanifold of $\reals^m$ determined by the system $Q_1(\bar{y})=\ldots = Q_r(\bar{y})=0$ is at most 
\[
    2^{q(q-1)/2}d_1\cdots d_r\cdot S^{m-r}\left[(m-r+1)S-(m-r)\right]^q
,
\]
where $S=mD+1+\sum_{i=1}^r(d_i-1)$.  
\end{lem}

So, let $(\bar{a}_1,c_1),\ldots, (\bar{a}_V,c_V)\in \reals^{n+1}$ be arbitrary and consider some subset of Pfaffian (so $C^\infty$) functions 
\[\tau_1(\bar{y}),\ldots, \tau_r(\bar{y})\in \{G(\bar{a}_i,\bar{y},c_i):1\leq i \leq V\}\] % Solved! \Bum{Index missing. $c$ should be $c_i$.}
where $r\leq p$. Let $\varepsilon_1,\ldots, \varepsilon_r\in \reals$ be arbitrary. We wish to unconditionally bound the number of connected components of the set 
\[\Xi^{-1}(\varepsilon_1,\ldots, \varepsilon_r) \eqdef \{\bar{y}\in\reals^p:\tau_i(\bar{y})=\varepsilon_i, 1\leq i\leq r\}\]

By Corollary \ref{cor:pfaff-substitution}, the $\tau_i(\bar{y}), 1\leq i \leq r$ are Pfaffian of degree at most $d$ over a \emph{common} chain of length $rq\leq pq$ and degree $D$. Consequently, the linear translates, $\chi_i(\bar{y}) \eqdef \tau_i(\bar{y})-\varepsilon_i$ are also Pfaffian of format at most $(rq, D, d)$ over a common chain. So, by Lemma~\ref{Kohv-bound}, 
\[\Xi^{-1}(\varepsilon_1,\ldots, \varepsilon_r) \eqdef \{\bar{y}\in\reals^p:\chi_i(\bar{y})=0, 1\leq i\leq r\}\]
is either empty, or has at most 
\[B\leq 2^{rq(rq-1)/2}d^r\cdot S^{p-r}\left[(p-r+1)S-(p-r)\right]^{rq}
,
\]
where $S=pD+1+r(d-1)$. Since $0\leq r\leq p$, we get an unconditional (worst-case) bound
\[B\leq 2^{pq(pq-1)/2}d^p\cdot [p(D+d-1)+1]^p[(p+1)(p(D+d-1)+1)]^{pq}.\]

Combining this bound with Lemma~\ref{KM-theorem} and Proposition \ref{prop:PNN_format} (for $s=1$, since we are only enlarging the language by one function) completes the proof of Theorem~\ref{thrm:PNNs}. 




\subsection{How Pfaffian Properties Preserve Complexity under Common Network Transformations}

Residual connections of the form \(x\mapsto \phi(x)+x\) are ubiquitous in modern deep architectures (ResNets~\cite{resnet}, Transformers~\cite{transformers}, etc.), since they improve gradient flow and ease optimization. From Lemma~\ref{pfaff-sum-format}, the following corollary on residual connections follows, which we will later use to analyze Transformer blocks.

\begin{cor}[Residual connections do not increase Pfaffian complexity]
\label{cor:residual-no-increase}
Let $\phi(\bar{x})$ be Pfaffian on a domain $U$ of format $(q,D,d)$, and let $\operatorname{Id}(\bar{x})=\bar{x}$ denote the identity map (a polynomial of degree $1$). Then the residual map
\[
\bar{x}\mapsto \phi(\bar{x})+\operatorname{Id}(\bar{x})
\]
is Pfaffian on $U$ of format at most $(q,D,\max\{d,1\})$. In particular, if $d\ge 1$ (which is the case for any non-constant polynomial representation of an activation), the format does not increase and the sum has format at most $(q,D,d)$.
\end{cor}

\begin{proof}
By Lemma~\ref{pfaff-sum-format}, adding the identity $\operatorname{Id}(\bar{x})=\bar{x}$ (format(0,0,1)) to $\phi(\bar{x})$ yields format $(q,\max\{D,0\},\max\{d,1\})=(q,D,\max\{d,1\})$, which equals $(q,D,d)$ whenever $d\ge 1$.
\end{proof}
\Bum{The statement writes the residual map $\bar x\mapsto \phi(\bar x)+\operatorname{Id}(\bar x)$ while only assuming that $\phi(\bar x)$ is Pfaffian on a domain $U$. Earlier closure lemmas are stated for scalar Pfaffian functions, and if $\phi:U\to\R$ while $\bar x\in\R^d$, then $\phi(\bar x)+\bar x$ is undefined. For the neural-network residual interpretation, one needs $\phi:U\to\R^d$. State the corollary componentwise. For example, if $\phi=(\phi_1,\dots,\phi_d):U\to\R^d$ and each $\phi_i$ is Pfaffian of format at most $(q,D,d)$ on $U$, then $\bar x\mapsto \phi(\bar x)+\bar x$ is Pfaffian componentwise with format at most $(q,D,\max\{d,1\})$.}

\begin{rmk}[Residuals with trainable scaling]
Including a trainable scalar multiplier $\gamma\in \mathbb{R}$ on the skip connection (which is less common in practice), i.e.\ $\phi(\bar{x})+\gamma \bar{x}$, also does not affect the format. The term $\gamma \bar{x}$ has degree $1$ in $\bar{x}$ (with $\gamma$ treated as a parameter). Therefore, the Pfaffian complexity remains unchanged.
\end{rmk}

\ocariz{Discuss gating}

\begin{cor}[Pfaffian functions under linear or affine maps]
\label{cor:linear-maps}
Let $\phi(\bar{x})$ be Pfaffian on a domain $U$ of format $(q,D,d)$, and let $L(\bar{x})=A\bar{x}+b$ be any fixed linear or affine map. Then the composition $\bar{x} \mapsto \phi(L(\bar{x}))$ is Pfaffian on $U$ of format at most $(q,D,d)$. That is, linear or affine maps do not increase Pfaffian complexity.
\end{cor}

\begin{proof}
Since $L(\bar{x})$ is a polynomial of degree $1$, composing $\phi$ with $L$ does not require additional chain elements or increase the algebraic degree of the polynomial representation in Definition~\ref{defn:PfaffianFunctionFormat}. By the standard closure properties of Pfaffian functions under composition with polynomials, the format remains $(q,D,d)$.
\end{proof}
\Bum{If $\phi$ is Pfaffian on a domain $U$ and $L(\bar{x})=A\bar{x}+b$, then $\phi(L(\bar{x}))$ is defined only for those $\bar{x}$ such that $L(\bar{x})\in U$. The current statement claims Pfaffianity on all of $U$, which need not be preserved by $L$. For example, if $U=(0,\infty)$, $\phi(u)=1/u$, and $L(x)=x-1$, then $\phi(L(x))$ is not defined on all of $U$. I would like to suggest writing the result on $L^{-1}(U)$. More generally, if $V$ is a domain with $L(V)\subseteq U$, then $\bar{x}\mapsto \phi(L(\bar{x}))$ is Pfaffian on $V$ with format at most $(q,D,d)$.}

\begin{rmk}[Linear projections in neural networks]
In most neural network architectures, each activation function is preceded by a linear projection, also known as a linear layer (e.g., in MLP layers or Transformer feedforward blocks). Corollary~\ref{cor:linear-maps} implies that these linear projections can be “absorbed” into the activation without increasing the Pfaffian complexity: the format $(q,D,d)$ of the activation remains valid for the composed map.
\end{rmk}


==> checklist.tex <==
\section*{NeurIPS Paper Checklist}




\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately state the paper's theoretical contribution and its scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper explicitly states that the results are qualitative, statistical, and limited to fixed finite feedforward architectures.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The assumptions are stated clearly and the main theoretical results are proved in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper is theoretical and does not include experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not rely on experimental code or datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include training or test experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not report empirical results requiring statistical significance analysis.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not include computational experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The work is foundational theory and does not involve human subjects, private data, or deployed systems.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper is foundational theoretical work with no direct application-specific societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not release high-risk data, models, or systems.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not use external datasets, code, or pretrained models as research assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not introduce or release new datasets, code, models, or benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve crowdsourcing or human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper does not involve human subjects, so IRB approval is not applicable.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLM is used only for writing, editing, or formatting purposes.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}
